Chow-Witt Rings of Classifying Spaces of Products of Multiplicative and Cyclic Groups

We compute the total Chow-Witt rings of the classifying space B\mu_n of the roots of unity, as well as the products BG_m x B\mu_n and B\mu_m x B\mu_n for all m,n greater than or equal to 1 based on the strategy by di Lorenzo and Mantovani (2023) for B\mu_n with n even. Moreover we compute the total I^j-cohomology and Chow-Witt rings of P^q x P^r for all q,r greater than or equal to 1 and of BG_m x BG_m.

==> commands.tex <==
\RequirePackage{mathtools}
\RequirePackage{amsmath, amssymb}
\RequirePackage{xcolor}
\RequirePackage{tikz}

%%%%%   TEXT FORMATTING   %%%%%

\newcommand{\defemph}{\textbf}

\newcommand{\todo}[1]{\textit{\color{red}[{#1}]}%\typeout{#1}
}\newcommand{\todominor}[1]{\textit{\color{orange}[{#1}]}%\typeout{#1}
}
\newcommand{\critical}{\marginpar{\Large\textbf{{\color{red}!!}}}}

%%%%% NUMBERS AND FIELDS %%%%%

\newcommand{\boldfont}{\mathbb}

\newcommand{\Gm}{\boldfont{G}_m}
\newcommand{\affine}{\mathbb{A}}
\newcommand{\Natural}{\boldfont{N}}
\newcommand{\Ibar}{\overline{I}}
\newcommand{\Ijcount}{c_{n,m,i,t}}
\newcommand{\Integer}{\boldfont{Z}}
\newcommand{\Rational}{\boldfont{Q}}
\newcommand{\Real}{\boldfont{R}}
\newcommand{\Complex}{\boldfont{C}}
\newcommand{\Finite}{\boldfont{F}}
\newcommand{\kf}{\boldfont{k}}
\newcommand{\Kf}{\boldfont{K}}
\newcommand{\Lf}{\boldfont{L}}
\newcommand{\projective}{\mathbb{P}}

%%%%% SPACES AND SCHEMES %%%%%
\newcommand{\Bmun}[2]{E_{#2}^{#1}}
\newcommand{\twist}[1]{\mathcal{O}{\if\relax\detokenize{#1}\relax\else{(#1)}\fi}}


%%%%% CATEGORIES %%%%%
\newcommand{\sslash}{/\mkern-6mu/}

\newcommand{\Anima}{\cat{An}}
\newcommand{\cat}[1]{\mathsf{#1}}
\newcommand{\CatInfty}{\cat{Cat}}
\newcommand{\CatStable}{\CatInfty^{\mathsf{st}}}
\DeclareMathOperator{\CGrp}{CGrp}
\DeclareMathOperator{\CMon}{CMon}
\newcommand{\completeSegal}{\cat{CS}}
\newcommand{\laxslice}[2]{#1_{/\mkern-4mu/#2}}
\newcommand{\presheaves}{\mathcal{P}}
\newcommand{\Set}{\cat{Set}}
\newcommand{\simplexcat}{
	\mathchoice{\Delta\llap{\scalebox{0.775}{$\Delta$\hspace{0.025em}}}}%
	{\Delta\llap{\scalebox{0.775}{$\Delta$\hspace{0.025em}}}}%
	{\Delta\llap{\scalebox{0.775}{$\scriptstyle\Delta$\hspace{0.025em}}}}%
	{\Delta\llap{\scalebox{0.775}{$\scriptscriptstyle\Delta$\hspace{0.025em}}}}
}
\newcommand{\slice}[2]{#1_{/#2}}
\newcommand{\Spectra}{\cat{Sp}}
\newcommand{\simplicial}{\cat{s}}

%%%%% OPERATORS %%%%%

\DeclareMathOperator{\Ar}{Ar}
\newcommand{\asscat}{B^{\mathrm{r}}}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\bockstein}{\beta}
\DeclareMathOperator{\bslice}{\slice{\mathcal{B}}{(-)}}
\DeclareMathOperator{\Center}{Z}
\DeclareMathOperator{\chern}{c}
\DeclareMathOperator{\chow}{CH}
\DeclareMathOperator{\chowmodtwo}{Ch}
\DeclareMathOperator{\chowwitt}{\widetilde{CH}}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\cofib}{cofib}
\DeclareMathOperator{\coker}{coker}
\newcommand{\colim}{\operatorname{colim}\displaylimits}
\DeclareMathOperator{\core}{core}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\dec}{d\'ec}
\renewcommand{\div}{\operatorname{div}}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\eulercw}{e} % Euler classes in Chow-Witt groups
\DeclareMathOperator{\euleri}{e} % Euler classes in I-cohomology
\DeclareMathOperator{\ev}{ev}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Exterior}{\bigwedge}
\DeclareMathOperator{\fib}{fib}
\DeclareMathOperator{\Fun}{Fun}
\DeclareMathOperator{\Funadd}{Fun^{add}}
\DeclareMathOperator{\Fungrp}{Fun^{grp}}
\DeclareMathOperator{\FunVerd}{Fun^{loc}}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\GW}{GW}
\DeclareMathOperator{\Hom}{Hom}
\newcommand{\ibar}{\overline{I}}
\DeclareMathOperator{\im}{im}
\newcommand{\KMW}{K^{\mathrm{MW}}}
\newcommand{\KM}{K^{\mathrm{M}}}
\newcommand{\KW}{K^{\mathrm{W}}}
\DeclareMathOperator{\Lan}{Lan}
\DeclareMathOperator{\Mat}{Mat}
\DeclareMathOperator{\modulo}{mod}
\DeclareMathOperator{\Mon}{Mon}
\DeclareMathOperator{\Nat}{Nat}
\DeclareMathOperator{\Null}{Null}
\DeclareMathOperator{\perf}{perf}
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\Ran}{Ran}
\DeclareMathOperator{\rank}{rk}
\newcommand{\relativeQ}{Q^{\mathrm{rel}}}
\newcommand{\rezkNerve}{N^{\mathrm{r}}}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\sw}{\overline{c}} %Stiefel-Whitney class
\DeclareMathOperator{\Symm}{S}
\DeclareMathOperator{\Tensor}{T}
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\transfer}{Tr}
\DeclareMathOperator{\twar}{TwAr}
\DeclareMathOperator{\unCart}{Un^{cart}}
\DeclareMathOperator{\unCocart}{Un^{cocart}}
\newcommand{\wbar}{\overline{W}}
\DeclareMathOperator{\witt}{W}



%%%%% FUNCTIONS %%%%%

\DeclareMathOperator{\ringchar}{char}
\newcommand{\esd}{\mathrm{esd}}
\newcommand{\forgetful}{\rho}
\newcommand{\hyperbolic}{h}
\newcommand{\id}{\mathrm{id}}
\newcommand{\pr}{\mathrm{pr}}
\newcommand{\reduction}{\widetilde{\rho}}
\newcommand{\sign}{sgn}
\DeclareMathOperator{\sqperiod}{\varphi}
\newcommand{\tr}{tr}



%%%%% SPECIAL ELEMENTS %%%%%

\newcommand{\cherna}{c_1}
\newcommand{\chernb}{c_2}
\newcommand{\eulercwz}{e}
\newcommand{\eulercwa}{\eulercwz_1}
\newcommand{\eulercwb}{\eulercwz_2}
\newcommand{\eulercwc}{\eulercwz_3}
\newcommand{\euleriz}{e}
\newcommand{\euleria}{\euleriz_1}
\newcommand{\eulerib}{\euleriz_2}
\newcommand{\euleric}{\euleriz_3}
\newcommand{\hyperbolicz}{H}
\newcommand{\hyperbolica}{H_1}
\newcommand{\hyperbolicb}{H_2}
\newcommand{\hyperbolicc}{H_3}
\newcommand{\orientationz}{R}
\newcommand{\orientationa}{R_1}
\newcommand{\orientationb}{R_2}
\newcommand{\swa}{\overline{c}_1}
\newcommand{\swb}{\overline{c}_2}
\newcommand{\vectorbundle}{E}
\newcommand{\vectorbundlesheaf}{\mathcal{E}}
\newcommand{\vectorbundleG}{G_E}
\newcommand{\vectorbundlesheafG}{\mathcal{G}_E}
\newcommand{\Id}{\mathbb{1}}
\newcommand{\linebundle}{\mathcal{L}}
\newcommand{\linebundleb}{\mathcal{M}}
\newcommand{\ph}{\mathrm{-}}
\newcommand{\phdot}{\,\cdot\,}
\newcommand{\trivialbundle}{\mathcal{O}}
\newcommand{\classu}{U}
\newcommand{\classua}{\classu_1}
\newcommand{\classub}{\classu_2}


%%%%% BINARY OPERATIONS %%%%%

\newcommand{\act}{\mathbin{.}}
\newcommand{\bigslant}[2]{{\raisebox{.2em}{$#1$}\left/\raisebox{-.2em}{$#2$}\right.}}
\newcommand{\tensor}{\otimes}
\newcommand{\join}{\mathbin{\star}}



%%%%% RELATIONS %%%%%

\newcommand{\defined}{\coloneqq}
\newcommand{\defines}{\eqqcolon}
\newcommand{\leftadjoint}{\dashv}
\newcommand{\rightadjoint}{\vdash}
\renewcommand{\setminus}{\smallsetminus}



%%%%% DELIMITERS %%%%%

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\class}{\lbrack}{\rbrack}
\DeclarePairedDelimiter{\ideal}{\lparen}{\rparen}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}



%%%%% DECORATIONS %%%%%

\newcommand{\ab}{\mathrm{ab}}
\newcommand{\conj}{\overline}
\newcommand{\induced}{\overline}
\newcommand{\op}{\mathrm{op}}
\newcommand{\sing}{\mathrm{sing}}
\newcommand{\tot}{{\tikz[baseline=-0.5ex]\draw[fill,radius=.3ex] (0,0) circle ;}} % total chow-witt ring
\newcommand{\trans}{\mathsf{t}}

% pushout and pullback symbols

\newcommand{\pullbacksign}{%
	\hspace{-0.25ex}%
	\tikz[baseline=(pb.base)]{%
		\draw[line width=rule_thickness, line cap=round]%
		(0,0)%
		++ (-0.5ex,-0.5ex)%
		-- ++(1ex,0ex)%
		-- ++ (0ex,1ex);%
		\filldraw (-0.3ex,0.3ex) circle (0.3pt);%
		\node (pb) at (0,0) {\phantom{x}};%
	}%
}
\newcommand{\pushoutsign}{%
	\hspace{0.25ex}%
	\tikz[baseline=(po.base)]{%
		\draw[line width=rule_thickness, line cap=round]%
		(0,0)%
		++ (-0.5ex,-0.5ex)%
		-- ++(0ex,1ex)%
		-- ++ (1ex,0ex);%
		\filldraw (0.3ex,-0.3ex) circle (0.3pt);%
		\node (po) at (0,0) {\phantom{x}};%
	}%
}
\tikzcdset{
	pullback/.style = {dash, phantom, "\pullbacksign", start anchor=center, end anchor=center},
	%	hpullback/.style = {dash, phantom, "\vphantom{x}\smash{\pullbacksign_{h}}", start anchor=center, end anchor=center},
	pushout/.style = {dash, phantom, "\pushoutsign", start anchor=center, end anchor=center}
}



%%%%% ARROWS %%%%%

\renewcommand{\to}{
	\mathchoice
	{\longrightarrow}
	{\rightarrow}
	{\rightarrow}
	{\rightarrow}
}
\newcommand{\from}{
	\mathchoice
	{\longleftarrow}
	{\leftarrow}
	{\leftarrow}
	{\leftarrow}
}
\AtBeginDocument{
	\let\oldmapsto\mapsto
	\renewcommand{\mapsto}{
		\mathchoice
		{\longmapsto}
		{\oldmapsto}
		{\oldmapsto}
		{\oldmapsto}
	}
}
%\AtBeginDocument{
%	\let\oldmapsfrom\mapsfrom
%	\renewcommand{\mapsfrom}{
%		\mathchoice
%		{\longmapsfrom}
%		{\oldmapsfrom}
%		{\oldmapsfrom}
%		{\oldmapsfrom}
%	}
%}
\newcommand{\onetoone}{
	\mathchoice
	{\longleftrightarrow}
	{\leftrightarrow}
	{\leftrightarrow}
	{\leftrightarrow}
}
\newcommand{\xto}[1]{
	\mathchoice
	{\xrightarrow{\enspace #1 \enspace}}
	{\xrightarrow{#1}}
	{\xrightarrow{#1}}
	{\xrightarrow{#1}}
}
\newcommand{\xfrom}[1]{
	\mathchoice
	{\xleftarrow{\enspace #1 \enspace}}
	{\xleftarrow{#1}}
	{\xleftarrow{#1}}
	{\xleftarrow{#1}}
}
%somewhat ugly
\NewDocumentCommand{\doublelrmorphism}{O{} O{}}{%
	\begin{tikzcd}[ampersand replacement=\&, cramped, column sep={\the\morphismlength-0.04em}]%
		\vphantom{x}\rar[shift left=0.45ex, "#1"]\& \lar[shift left=0.45ex, "#2"] \vphantom{x}%
	\end{tikzcd}%
}



%%%%% MISC %%%%%

% cocolon for writing functors from right to left
\newcommand*{\cocolon}{%
	\nobreak
	\mskip6mu plus1mu
	\mathpunct{}%
	\nonscript
	\mkern-\thinmuskip
	{:}%
	\mskip2mu
	\relax
}

% iddots
\newcommand{\iddots}{⋰}

% larger bullet
\let\oldbullet\bullet
\renewcommand{\bullet}{{\scalebox{1.15}{\oldbullet}}}

% restrict{f}{X} for f|_X
% restrict[Y]{f}{X} for f
% stared version scales the delimiter
% restrict[\(bB)ig(g)] for manual scaling of the delimiter
% * has precedent over manual scaling if both are given
\DeclarePairedDelimiter{\prerestrict}{.}{\rvert} % period = empty delimiter
\NewDocumentCommand%
{\restrict}%
{s o m m O{}}%
{%
	\IfBooleanTF{#1}
	{%
		\prerestrict*{#3}_{#4}^{5}
	}
	{%
		\IfValueTF{#2}
		{%
			\prerestrict[#2]{#3}_{#4}^{5}
		}
		{%
			#3\rvert_{#4}^{5}
		}
	}
}

% \suchthat for inline
% \suchthat* for for display math with \left and \right
% \suchthat[\(bB)ig(g)] for manual scaling in display math
\NewDocumentCommand%
{\suchthat}%
{so}
{%
	\IfValueTF{#2}
	{%
		\:#2|\:
	}
	{%
		\IfBooleanTF{#1}
		{%
			\:\middle|\:
		}
		{%
			\mathrel{|}
		}
	}
}


